Demand forecasting techniques for build-to-order lean manufacturing supply chains

Build-to-order (BTO) supply chains have become common-place in industries such as electronics, automotive and fashion. They enable building products based on individual requirements with a short lead time and minimum inventory and production costs. Due to their nature, they differ significantly from traditional supply chains. However, there have not been studies dedicated to demand forecasting methods for this type of setting. This work makes two contributions. First, it presents a new and unique data set from a manufacturer in the BTO sector. Second, it proposes a novel data transformation technique for demand forecasting of BTO products. Results from thirteen forecasting methods show that the approach compares well to the state-of-the-art while being easy to implement and to explain to decision-makers.

==> figures/graph.tex <==
\begin{tikzpicture}[scale=0.5]
    \begin{scope}[every node/.style={circle,thin,draw,scale=0.60}]
        \node (A) at (1.25, 0.00) {1};
        \node (C) at (1.00, 3.00) {2};
        \node (G) at (0.50, 1.50) {3};
        \node (F) at (4.00, 3.00) {4};
        \node (D) at (4.25, 1.00) {5};
        \node (M) at (4.50,-0.25) {6};
        \node (H) at (6.50, 0.50) {7};
        \node (J) at (6.00, 2.50) {8};
        \node (N) at (5.50,-0.50) {9};
    \end{scope}
    \begin{scope}[
        every node/.style={fill=white,circle},
        every edge/.style={draw=red,very thick}]
        \draw (A) -> (G);
        \draw (G) -> (C);
        \draw (H) -> (J);
        \draw (N) -> (H);
    
        \draw (G) -> (D);
        \draw (G) -> (F);
        \draw (C) -> (F);
        \draw (C) -> (M);
        \draw (N) -> (F);
        \draw (N) -> (M);
        \draw (J) -> (D);
        \draw (J) -> (F);
        \draw (H) -> (F);
    \end{scope}
\end{tikzpicture}

==> figures/sparse_mf.tex <==
\begin{tikzpicture}[scale=0.5]
    \draw[step=0.2,gray!50,thin] (0.0, 0.0) grid (5.0, 7.0);
    % random_state = np.random.RandomState(0x0BADCAFE)
    % h, w, step = 7.0, 5.0, 0.2
    
    % xx, yy = np.meshgrid(np.r_[0:w:step], np.r_[0:h:step])
    % n_obs = np.prod(xx.shape)
    % coord = random_state.choice(n_obs, size=int(n_obs * 0.25), replace=False)
    % coord = np.sort(coord)
    % ii, jj = np.unravel_index(coord, xx.shape)
    
    % observed = []
    % for i, j in zip(ii, jj):
    %     x, y = xx[i, j], yy[i, j]
    %     observed.append(r"""\filldraw[fill=black!30!white, draw=none]"""
    %                   f""" ({x:.1f}, {y:.1f}) rectangle"""
    %                   f""" ({x + step:.1f}, {y + step:.1f});""")
    
    % print("\n".join(observed))
    {
        \filldraw[fill=black!30!white, draw=none] (0.0, 0.0) rectangle (0.2, 0.2);
        \filldraw[fill=black!30!white, draw=none] (0.4, 0.0) rectangle (0.6, 0.2);
        \filldraw[fill=black!30!white, draw=none] (0.6, 0.0) rectangle (0.8, 0.2);
        \filldraw[fill=black!30!white, draw=none] (0.8, 0.0) rectangle (1.0, 0.2);
        \filldraw[fill=black!30!white, draw=none] (1.0, 0.0) rectangle (1.2, 0.2);
        \filldraw[fill=black!30!white, draw=none] (1.8, 0.0) rectangle (2.0, 0.2);
        \filldraw[fill=black!30!white, draw=none] (2.8, 0.0) rectangle (3.0, 0.2);
        \filldraw[fill=black!30!white, draw=none] (3.4, 0.0) rectangle (3.6, 0.2);
        \filldraw[fill=black!30!white, draw=none] (4.0, 0.0) rectangle (4.2, 0.2);
        \filldraw[fill=black!30!white, draw=none] (4.2, 0.0) rectangle (4.4, 0.2);
        \filldraw[fill=black!30!white, draw=none] (0.2, 0.2) rectangle (0.4, 0.4);
        \filldraw[fill=black!30!white, draw=none] (1.2, 0.2) rectangle (1.4, 0.4);
        \filldraw[fill=black!30!white, draw=none] (2.2, 0.2) rectangle (2.4, 0.4);
        \filldraw[fill=black!30!white, draw=none] (2.4, 0.2) rectangle (2.6, 0.4);
        \filldraw[fill=black!30!white, draw=none] (2.8, 0.2) rectangle (3.0, 0.4);
        \filldraw[fill=black!30!white, draw=none] (4.4, 0.2) rectangle (4.6, 0.4);
        \filldraw[fill=black!30!white, draw=none] (1.6, 0.4) rectangle (1.8, 0.6);
        \filldraw[fill=black!30!white, draw=none] (2.6, 0.4) rectangle (2.8, 0.6);
        \filldraw[fill=black!30!white, draw=none] (3.6, 0.4) rectangle (3.8, 0.6);
        \filldraw[fill=black!30!white, draw=none] (4.2, 0.4) rectangle (4.4, 0.6);
        \filldraw[fill=black!30!white, draw=none] (4.4, 0.4) rectangle (4.6, 0.6);
        \filldraw[fill=black!30!white, draw=none] (4.6, 0.4) rectangle (4.8, 0.6);
        \filldraw[fill=black!30!white, draw=none] (0.8, 0.6) rectangle (1.0, 0.8);
        \filldraw[fill=black!30!white, draw=none] (1.4, 0.6) rectangle (1.6, 0.8);
        \filldraw[fill=black!30!white, draw=none] (1.8, 0.6) rectangle (2.0, 0.8);
        \filldraw[fill=black!30!white, draw=none] (2.0, 0.6) rectangle (2.2, 0.8);
        \filldraw[fill=black!30!white, draw=none] (2.4, 0.6) rectangle (2.6, 0.8);
        \filldraw[fill=black!30!white, draw=none] (3.0, 0.6) rectangle (3.2, 0.8);
        \filldraw[fill=black!30!white, draw=none] (4.2, 0.6) rectangle (4.4, 0.8);
        \filldraw[fill=black!30!white, draw=none] (4.4, 0.6) rectangle (4.6, 0.8);
        \filldraw[fill=black!30!white, draw=none] (2.0, 0.8) rectangle (2.2, 1.0);
        \filldraw[fill=black!30!white, draw=none] (2.2, 0.8) rectangle (2.4, 1.0);
        \filldraw[fill=black!30!white, draw=none] (2.6, 0.8) rectangle (2.8, 1.0);
        \filldraw[fill=black!30!white, draw=none] (2.8, 0.8) rectangle (3.0, 1.0);
        \filldraw[fill=black!30!white, draw=none] (4.6, 0.8) rectangle (4.8, 1.0);
        \filldraw[fill=black!30!white, draw=none] (0.0, 1.0) rectangle (0.2, 1.2);
        \filldraw[fill=black!30!white, draw=none] (3.6, 1.0) rectangle (3.8, 1.2);
        \filldraw[fill=black!30!white, draw=none] (4.6, 1.0) rectangle (4.8, 1.2);
        \filldraw[fill=black!30!white, draw=none] (0.8, 1.2) rectangle (1.0, 1.4);
        \filldraw[fill=black!30!white, draw=none] (1.4, 1.2) rectangle (1.6, 1.4);
        \filldraw[fill=black!30!white, draw=none] (3.6, 1.2) rectangle (3.8, 1.4);
        \filldraw[fill=black!30!white, draw=none] (4.2, 1.2) rectangle (4.4, 1.4);
        \filldraw[fill=black!30!white, draw=none] (0.0, 1.4) rectangle (0.2, 1.6);
        \filldraw[fill=black!30!white, draw=none] (0.4, 1.4) rectangle (0.6, 1.6);
        \filldraw[fill=black!30!white, draw=none] (3.4, 1.4) rectangle (3.6, 1.6);
        \filldraw[fill=black!30!white, draw=none] (0.4, 1.6) rectangle (0.6, 1.8);
        \filldraw[fill=black!30!white, draw=none] (1.2, 1.6) rectangle (1.4, 1.8);
        \filldraw[fill=black!30!white, draw=none] (1.4, 1.6) rectangle (1.6, 1.8);
        \filldraw[fill=black!30!white, draw=none] (1.6, 1.6) rectangle (1.8, 1.8);
        \filldraw[fill=black!30!white, draw=none] (2.0, 1.6) rectangle (2.2, 1.8);
        \filldraw[fill=black!30!white, draw=none] (2.8, 1.6) rectangle (3.0, 1.8);
        \filldraw[fill=black!30!white, draw=none] (4.2, 1.6) rectangle (4.4, 1.8);
        \filldraw[fill=black!30!white, draw=none] (4.8, 1.6) rectangle (5.0, 1.8);
        \filldraw[fill=black!30!white, draw=none] (0.6, 1.8) rectangle (0.8, 2.0);
        \filldraw[fill=black!30!white, draw=none] (1.8, 1.8) rectangle (2.0, 2.0);
        \filldraw[fill=black!30!white, draw=none] (2.8, 1.8) rectangle (3.0, 2.0);
        \filldraw[fill=black!30!white, draw=none] (3.6, 1.8) rectangle (3.8, 2.0);
        \filldraw[fill=black!30!white, draw=none] (4.8, 1.8) rectangle (5.0, 2.0);
        \filldraw[fill=black!30!white, draw=none] (1.0, 2.0) rectangle (1.2, 2.2);
        \filldraw[fill=black!30!white, draw=none] (1.2, 2.0) rectangle (1.4, 2.2);
        \filldraw[fill=black!30!white, draw=none] (1.8, 2.0) rectangle (2.0, 2.2);
        \filldraw[fill=black!30!white, draw=none] (2.2, 2.0) rectangle (2.4, 2.2);
        \filldraw[fill=black!30!white, draw=none] (2.4, 2.0) rectangle (2.6, 2.2);
        \filldraw[fill=black!30!white, draw=none] (3.8, 2.0) rectangle (4.0, 2.2);
        \filldraw[fill=black!30!white, draw=none] (0.0, 2.2) rectangle (0.2, 2.4);
        \filldraw[fill=black!30!white, draw=none] (0.6, 2.2) rectangle (0.8, 2.4);
        \filldraw[fill=black!30!white, draw=none] (1.2, 2.2) rectangle (1.4, 2.4);
        \filldraw[fill=black!30!white, draw=none] (3.0, 2.2) rectangle (3.2, 2.4);
        \filldraw[fill=black!30!white, draw=none] (3.8, 2.2) rectangle (4.0, 2.4);
        \filldraw[fill=black!30!white, draw=none] (4.0, 2.2) rectangle (4.2, 2.4);
        \filldraw[fill=black!30!white, draw=none] (0.8, 2.4) rectangle (1.0, 2.6);
        \filldraw[fill=black!30!white, draw=none] (1.2, 2.4) rectangle (1.4, 2.6);
        \filldraw[fill=black!30!white, draw=none] (3.2, 2.4) rectangle (3.4, 2.6);
        \filldraw[fill=black!30!white, draw=none] (3.8, 2.4) rectangle (4.0, 2.6);
        \filldraw[fill=black!30!white, draw=none] (4.0, 2.4) rectangle (4.2, 2.6);
        \filldraw[fill=black!30!white, draw=none] (0.8, 2.6) rectangle (1.0, 2.8);
        \filldraw[fill=black!30!white, draw=none] (2.0, 2.6) rectangle (2.2, 2.8);
        \filldraw[fill=black!30!white, draw=none] (2.6, 2.6) rectangle (2.8, 2.8);
        \filldraw[fill=black!30!white, draw=none] (2.8, 2.6) rectangle (3.0, 2.8);
        \filldraw[fill=black!30!white, draw=none] (4.0, 2.6) rectangle (4.2, 2.8);
        \filldraw[fill=black!30!white, draw=none] (4.2, 2.6) rectangle (4.4, 2.8);
        \filldraw[fill=black!30!white, draw=none] (0.6, 2.8) rectangle (0.8, 3.0);
        \filldraw[fill=black!30!white, draw=none] (1.2, 2.8) rectangle (1.4, 3.0);
        \filldraw[fill=black!30!white, draw=none] (1.8, 2.8) rectangle (2.0, 3.0);
        \filldraw[fill=black!30!white, draw=none] (2.2, 2.8) rectangle (2.4, 3.0);
        \filldraw[fill=black!30!white, draw=none] (3.2, 2.8) rectangle (3.4, 3.0);
        \filldraw[fill=black!30!white, draw=none] (3.4, 2.8) rectangle (3.6, 3.0);
        \filldraw[fill=black!30!white, draw=none] (4.4, 2.8) rectangle (4.6, 3.0);
        \filldraw[fill=black!30!white, draw=none] (4.8, 2.8) rectangle (5.0, 3.0);
        \filldraw[fill=black!30!white, draw=none] (0.6, 3.0) rectangle (0.8, 3.2);
        \filldraw[fill=black!30!white, draw=none] (1.6, 3.0) rectangle (1.8, 3.2);
        \filldraw[fill=black!30!white, draw=none] (2.2, 3.0) rectangle (2.4, 3.2);
        \filldraw[fill=black!30!white, draw=none] (2.8, 3.0) rectangle (3.0, 3.2);
        \filldraw[fill=black!30!white, draw=none] (3.0, 3.0) rectangle (3.2, 3.2);
        \filldraw[fill=black!30!white, draw=none] (3.2, 3.0) rectangle (3.4, 3.2);
        \filldraw[fill=black!30!white, draw=none] (3.6, 3.0) rectangle (3.8, 3.2);
        \filldraw[fill=black!30!white, draw=none] (4.2, 3.0) rectangle (4.4, 3.2);
        \filldraw[fill=black!30!white, draw=none] (0.8, 3.2) rectangle (1.0, 3.4);
        \filldraw[fill=black!30!white, draw=none] (1.0, 3.2) rectangle (1.2, 3.4);
        \filldraw[fill=black!30!white, draw=none] (1.6, 3.2) rectangle (1.8, 3.4);
        \filldraw[fill=black!30!white, draw=none] (2.0, 3.2) rectangle (2.2, 3.4);
        \filldraw[fill=black!30!white, draw=none] (2.6, 3.2) rectangle (2.8, 3.4);
        \filldraw[fill=black!30!white, draw=none] (3.0, 3.2) rectangle (3.2, 3.4);
        \filldraw[fill=black!30!white, draw=none] (3.2, 3.2) rectangle (3.4, 3.4);
        \filldraw[fill=black!30!white, draw=none] (3.4, 3.2) rectangle (3.6, 3.4);
        \filldraw[fill=black!30!white, draw=none] (4.0, 3.2) rectangle (4.2, 3.4);
        \filldraw[fill=black!30!white, draw=none] (4.8, 3.2) rectangle (5.0, 3.4);
        \filldraw[fill=black!30!white, draw=none] (1.0, 3.4) rectangle (1.2, 3.6);
        \filldraw[fill=black!30!white, draw=none] (1.8, 3.4) rectangle (2.0, 3.6);
        \filldraw[fill=black!30!white, draw=none] (2.2, 3.4) rectangle (2.4, 3.6);
        \filldraw[fill=black!30!white, draw=none] (2.6, 3.4) rectangle (2.8, 3.6);
        \filldraw[fill=black!30!white, draw=none] (3.4, 3.4) rectangle (3.6, 3.6);
        \filldraw[fill=black!30!white, draw=none] (3.8, 3.4) rectangle (4.0, 3.6);
        \filldraw[fill=black!30!white, draw=none] (0.6, 3.6) rectangle (0.8, 3.8);
        \filldraw[fill=black!30!white, draw=none] (1.2, 3.6) rectangle (1.4, 3.8);
        \filldraw[fill=black!30!white, draw=none] (2.0, 3.6) rectangle (2.2, 3.8);
        \filldraw[fill=black!30!white, draw=none] (2.4, 3.6) rectangle (2.6, 3.8);
        \filldraw[fill=black!30!white, draw=none] (2.6, 3.6) rectangle (2.8, 3.8);
        \filldraw[fill=black!30!white, draw=none] (3.2, 3.6) rectangle (3.4, 3.8);
        \filldraw[fill=black!30!white, draw=none] (3.4, 3.6) rectangle (3.6, 3.8);
        \filldraw[fill=black!30!white, draw=none] (1.0, 3.8) rectangle (1.2, 4.0);
        \filldraw[fill=black!30!white, draw=none] (1.2, 3.8) rectangle (1.4, 4.0);
        \filldraw[fill=black!30!white, draw=none] (1.4, 3.8) rectangle (1.6, 4.0);
        \filldraw[fill=black!30!white, draw=none] (1.6, 3.8) rectangle (1.8, 4.0);
        \filldraw[fill=black!30!white, draw=none] (2.6, 3.8) rectangle (2.8, 4.0);
        \filldraw[fill=black!30!white, draw=none] (3.0, 3.8) rectangle (3.2, 4.0);
        \filldraw[fill=black!30!white, draw=none] (3.4, 3.8) rectangle (3.6, 4.0);
        \filldraw[fill=black!30!white, draw=none] (3.6, 3.8) rectangle (3.8, 4.0);
        \filldraw[fill=black!30!white, draw=none] (3.8, 3.8) rectangle (4.0, 4.0);
        \filldraw[fill=black!30!white, draw=none] (4.2, 3.8) rectangle (4.4, 4.0);
        \filldraw[fill=black!30!white, draw=none] (4.4, 3.8) rectangle (4.6, 4.0);
        \filldraw[fill=black!30!white, draw=none] (0.4, 4.0) rectangle (0.6, 4.2);
        \filldraw[fill=black!30!white, draw=none] (1.6, 4.0) rectangle (1.8, 4.2);
        \filldraw[fill=black!30!white, draw=none] (3.2, 4.0) rectangle (3.4, 4.2);
        \filldraw[fill=black!30!white, draw=none] (3.4, 4.0) rectangle (3.6, 4.2);
        \filldraw[fill=black!30!white, draw=none] (3.6, 4.0) rectangle (3.8, 4.2);
        \filldraw[fill=black!30!white, draw=none] (4.0, 4.0) rectangle (4.2, 4.2);
        \filldraw[fill=black!30!white, draw=none] (1.2, 4.2) rectangle (1.4, 4.4);
        \filldraw[fill=black!30!white, draw=none] (1.6, 4.2) rectangle (1.8, 4.4);
        \filldraw[fill=black!30!white, draw=none] (2.0, 4.2) rectangle (2.2, 4.4);
        \filldraw[fill=black!30!white, draw=none] (2.4, 4.2) rectangle (2.6, 4.4);
        \filldraw[fill=black!30!white, draw=none] (4.0, 4.2) rectangle (4.2, 4.4);
        \filldraw[fill=black!30!white, draw=none] (4.2, 4.2) rectangle (4.4, 4.4);
        \filldraw[fill=black!30!white, draw=none] (4.4, 4.2) rectangle (4.6, 4.4);
        \filldraw[fill=black!30!white, draw=none] (0.6, 4.4) rectangle (0.8, 4.6);
        \filldraw[fill=black!30!white, draw=none] (0.8, 4.4) rectangle (1.0, 4.6);
        \filldraw[fill=black!30!white, draw=none] (1.4, 4.4) rectangle (1.6, 4.6);
        \filldraw[fill=black!30!white, draw=none] (3.4, 4.4) rectangle (3.6, 4.6);
        \filldraw[fill=black!30!white, draw=none] (4.0, 4.4) rectangle (4.2, 4.6);
        \filldraw[fill=black!30!white, draw=none] (4.6, 4.4) rectangle (4.8, 4.6);
        \filldraw[fill=black!30!white, draw=none] (0.0, 4.6) rectangle (0.2, 4.8);
        \filldraw[fill=black!30!white, draw=none] (1.6, 4.6) rectangle (1.8, 4.8);
        \filldraw[fill=black!30!white, draw=none] (1.8, 4.6) rectangle (2.0, 4.8);
        \filldraw[fill=black!30!white, draw=none] (2.6, 4.6) rectangle (2.8, 4.8);
        \filldraw[fill=black!30!white, draw=none] (0.6, 4.8) rectangle (0.8, 5.0);
        \filldraw[fill=black!30!white, draw=none] (1.0, 4.8) rectangle (1.2, 5.0);
        \filldraw[fill=black!30!white, draw=none] (1.8, 4.8) rectangle (2.0, 5.0);
        \filldraw[fill=black!30!white, draw=none] (2.8, 4.8) rectangle (3.0, 5.0);
        \filldraw[fill=black!30!white, draw=none] (3.8, 4.8) rectangle (4.0, 5.0);
        \filldraw[fill=black!30!white, draw=none] (4.6, 4.8) rectangle (4.8, 5.0);
        \filldraw[fill=black!30!white, draw=none] (1.0, 5.0) rectangle (1.2, 5.2);
        \filldraw[fill=black!30!white, draw=none] (1.6, 5.0) rectangle (1.8, 5.2);
        \filldraw[fill=black!30!white, draw=none] (2.2, 5.0) rectangle (2.4, 5.2);
        \filldraw[fill=black!30!white, draw=none] (2.4, 5.0) rectangle (2.6, 5.2);
        \filldraw[fill=black!30!white, draw=none] (3.6, 5.0) rectangle (3.8, 5.2);
        \filldraw[fill=black!30!white, draw=none] (4.0, 5.0) rectangle (4.2, 5.2);
        \filldraw[fill=black!30!white, draw=none] (4.6, 5.0) rectangle (4.8, 5.2);
        \filldraw[fill=black!30!white, draw=none] (1.0, 5.2) rectangle (1.2, 5.4);
        \filldraw[fill=black!30!white, draw=none] (1.2, 5.2) rectangle (1.4, 5.4);
        \filldraw[fill=black!30!white, draw=none] (1.4, 5.2) rectangle (1.6, 5.4);
        \filldraw[fill=black!30!white, draw=none] (1.8, 5.2) rectangle (2.0, 5.4);
        \filldraw[fill=black!30!white, draw=none] (2.2, 5.2) rectangle (2.4, 5.4);
        \filldraw[fill=black!30!white, draw=none] (3.0, 5.2) rectangle (3.2, 5.4);
        \filldraw[fill=black!30!white, draw=none] (3.4, 5.2) rectangle (3.6, 5.4);
        \filldraw[fill=black!30!white, draw=none] (0.6, 5.4) rectangle (0.8, 5.6);
        \filldraw[fill=black!30!white, draw=none] (2.0, 5.4) rectangle (2.2, 5.6);
        \filldraw[fill=black!30!white, draw=none] (2.2, 5.4) rectangle (2.4, 5.6);
        \filldraw[fill=black!30!white, draw=none] (2.8, 5.4) rectangle (3.0, 5.6);
        \filldraw[fill=black!30!white, draw=none] (3.0, 5.4) rectangle (3.2, 5.6);
        \filldraw[fill=black!30!white, draw=none] (3.4, 5.4) rectangle (3.6, 5.6);
        \filldraw[fill=black!30!white, draw=none] (4.2, 5.4) rectangle (4.4, 5.6);
        \filldraw[fill=black!30!white, draw=none] (4.8, 5.4) rectangle (5.0, 5.6);
        \filldraw[fill=black!30!white, draw=none] (0.6, 5.6) rectangle (0.8, 5.8);
        \filldraw[fill=black!30!white, draw=none] (0.8, 5.6) rectangle (1.0, 5.8);
        \filldraw[fill=black!30!white, draw=none] (1.2, 5.6) rectangle (1.4, 5.8);
        \filldraw[fill=black!30!white, draw=none] (2.0, 5.6) rectangle (2.2, 5.8);
        \filldraw[fill=black!30!white, draw=none] (3.0, 5.6) rectangle (3.2, 5.8);
        \filldraw[fill=black!30!white, draw=none] (4.6, 5.6) rectangle (4.8, 5.8);
        \filldraw[fill=black!30!white, draw=none] (4.8, 5.6) rectangle (5.0, 5.8);
        \filldraw[fill=black!30!white, draw=none] (1.0, 5.8) rectangle (1.2, 6.0);
        \filldraw[fill=black!30!white, draw=none] (1.8, 5.8) rectangle (2.0, 6.0);
        \filldraw[fill=black!30!white, draw=none] (2.2, 5.8) rectangle (2.4, 6.0);
        \filldraw[fill=black!30!white, draw=none] (3.6, 5.8) rectangle (3.8, 6.0);
        \filldraw[fill=black!30!white, draw=none] (4.0, 5.8) rectangle (4.2, 6.0);
        \filldraw[fill=black!30!white, draw=none] (4.4, 5.8) rectangle (4.6, 6.0);
        \filldraw[fill=black!30!white, draw=none] (1.0, 6.0) rectangle (1.2, 6.2);
        \filldraw[fill=black!30!white, draw=none] (4.0, 6.0) rectangle (4.2, 6.2);
        \filldraw[fill=black!30!white, draw=none] (4.2, 6.0) rectangle (4.4, 6.2);
        \filldraw[fill=black!30!white, draw=none] (0.6, 6.2) rectangle (0.8, 6.4);
        \filldraw[fill=black!30!white, draw=none] (0.8, 6.2) rectangle (1.0, 6.4);
        \filldraw[fill=black!30!white, draw=none] (2.0, 6.2) rectangle (2.2, 6.4);
        \filldraw[fill=black!30!white, draw=none] (2.2, 6.2) rectangle (2.4, 6.4);
        \filldraw[fill=black!30!white, draw=none] (4.2, 6.2) rectangle (4.4, 6.4);
        \filldraw[fill=black!30!white, draw=none] (4.4, 6.2) rectangle (4.6, 6.4);
        \filldraw[fill=black!30!white, draw=none] (1.0, 6.4) rectangle (1.2, 6.6);
        \filldraw[fill=black!30!white, draw=none] (2.4, 6.4) rectangle (2.6, 6.6);
        \filldraw[fill=black!30!white, draw=none] (2.8, 6.4) rectangle (3.0, 6.6);
        \filldraw[fill=black!30!white, draw=none] (3.2, 6.4) rectangle (3.4, 6.6);
        \filldraw[fill=black!30!white, draw=none] (4.0, 6.4) rectangle (4.2, 6.6);
        \filldraw[fill=black!30!white, draw=none] (2.4, 6.6) rectangle (2.6, 6.8);
        \filldraw[fill=black!30!white, draw=none] (2.8, 6.6) rectangle (3.0, 6.8);
        \filldraw[fill=black!30!white, draw=none] (0.0, 6.8) rectangle (0.2, 7.0);
        \filldraw[fill=black!30!white, draw=none] (1.4, 6.8) rectangle (1.6, 7.0);
        \filldraw[fill=black!30!white, draw=none] (2.0, 6.8) rectangle (2.2, 7.0);
        \filldraw[fill=black!30!white, draw=none] (3.2, 6.8) rectangle (3.4, 7.0);
        \filldraw[fill=black!30!white, draw=none] (4.2, 6.8) rectangle (4.4, 7.0);
        \filldraw[fill=black!30!white, draw=none] (4.4, 6.8) rectangle (4.6, 7.0);
        \filldraw[fill=black!30!white, draw=none] (4.6, 6.8) rectangle (4.8, 7.0);
    }
    
    \draw[thick] (0.0, 0.0) rectangle (5.0, 7.0) node[midway] {$\mathbf{Y}$};
    
    \node at (5.5, 3.5)  {$\mathbf{\approx}$};
    
    \draw[thick,fill=orange!30!white] (6.0, 0.0) rectangle (7.5, 7.0) node[midway] {$X$};
    \node at (8.0, 6.25)  {$\mathbf{\times}$};
    \draw[thick,fill=gray!30!white] (8.5, 5.5) rectangle (13.5, 7.0) node[midway] {$F$};
\end{tikzpicture}

==> figures/trmf_forecast.tex <==

\begin{tikzpicture}[scale=0.40]
    \draw[thick,fill=gray!30!white] (10, -1.5) rectangle (15, 0.0) node[midway] {$F$};
    \node at (12.5, 0.65) {\small{objects}};
    
    \draw[thick,fill=orange!30!white] (7, 1) rectangle (9, 4) node[midway] {$X$};
    \node[rotate=90] at (6.0, 2.50) {\small{time}};
    \path[draw,thin,->] (6.5, 3.75) -- (6.5, 1.25);
    
    \draw[thick,fill=green!30!white] (7.0, -1.5) rectangle (9, 0)
        node[midway] {\small{$\hat{X}_{T+h\mid T}$}};
    
    \draw[thick,fill=green!30!white] (0, -1.5) rectangle (5, 0)
        node[midway] {\small{$\hat{Y}_{T+h\mid T}$}};
    
    \node at (9.5, -0.75)  {$\mathbf{\times}$};
    \draw[thick,->] (8, 2) -- (8, -0.5);
    \node at (6.0, -0.75)  {$\mathbf{\longleftarrow}$};
\end{tikzpicture}
